INSPECTRE: Privately Estimating the Unseen

We develop differentially private methods for estimating various distributional properties. Given a sample from a discrete distribution $p$, some functional $f$, and accuracy and privacy parameters $\alpha$ and $\varepsilon$, the goal is to estimate $f(p)$ up to accuracy $\alpha$, while maintaining $\varepsilon$-differential privacy of the sample. We prove almost-tight bounds on the sample size required for this problem for several functionals of interest, including support size, support coverage, and entropy. We show that the cost of privacy is negligible in a variety of settings, both theoretically and experimentally. Our methods are based on a sensitivity analysis of several state-of-the-art methods for estimating these properties with sublinear sample complexities.

==> empirical.tex <==
\subsubsection{Upper Bound for Entropy Estimation: The Empirical Estimator}
\label{sec:entropy-ub-empirical}


Let $\emp$ be the empirical distribution, and let $\entemp$ be the entropy of the empirical distribution.

\begin{theorem}\label{thm:empirical}
\[
C(H, \dist, \eps) = O\Paren{\frac{\ab}{\dist}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2}+\frac{1}{\dist\eps}\log\Paren{\frac1{\dist\eps}}}.
\]
\end{theorem}

\begin{proof}
We present the entire argument for completeness. We will show that the theorem is implied by the following three results. 
\begin{align}
&\absv{\entp{\p}-\expectation{\entemp}} =O\Paren{\frac{\ab}{\ns}},\label{eq:bias-emp}\\
&\variance{\entemp} =O\Paren{\frac{\log^2(\min\{\ab,\ns\})}{\ns}},\label{eq:variance-emp}\\
&\Delta(\entemp) = O\Paren{\frac{\log\ns}{\ns}}.\label{eqn:sensitivity-emp}
\end{align}
Using these three equations, we are done.
\end{proof}

\paragraph{Proof of~\eqref{eq:bias-emp}.} By the concavity of entropy function, we know that 
\[
\expectation{\entp{\emp}} \le \entp{\p}.
\]
Therefore, 
\begin{align}
\expectation{\absv{\entp{\p}-\entp{\emp}}} &=  \entp{\p}-\expectation{{\entp{\emp}}}\nonumber\\
&=  \expectation{\sum_{\smb}\Paren{\pemps\log \pemps-\ps\log\ps}} \nonumber\\
&=  \expectation{\sum_{\smb}\pemps\log \frac{\pemps}{\ps}}+\expectation{\sum_{\smb}(\pemps-\ps)\log\ps}\nonumber\\
&=  \expectation{\kldist{\emp}{\p}}\label{eqn:kl-exp}\\
&\leq \expectation{\chisquare{\emp}{\p}}\label{eqn:kl-chisq}\\
&=  \expectation{\sum_{\smb}\frac{(\pemps-\ps)^2}{\ps}}\nonumber\\
&\le  {\sum_{\smb}\frac{(\ps/\ns)}{\ps}}\label{eqn:var-bin}\\
&= \frac\ab\ns.
\end{align}

\paragraph{Proof of~\eqref{eqn:sensitivity-emp}.}
The largest change in any $\nsmb$ when we change one symbol is one. Moreover, at most two $\nsmb$ changes. Therefore, 
\begin{align}
\Delta(\entemp) &\leq  2\cdot \max_{j=1\ldots \ns-1} \absv{ \frac{j+1}{n}\log\frac{n}{j+1}-\frac{j}{n}\log\frac{n}{j}}\nonumber\\
&=  2\cdot \max_{j=1\ldots \ns-1}\absv{\frac{j}{\ns}\log \frac{j}{j+1}+\frac1{\ns}\log \frac{\ns}{j+1}}\label{eqn:sum-one}\\
&\leq  2 \cdot \max_{j=1\ldots \ns-1}\max\left\{\absv{\frac{j}{\ns}\log \frac{j}{j+1}}, \absv{ \frac1{\ns}\log \frac{\ns}{j+1}}\right\}\label{eqn:sum-two}\\
&\leq  2\cdot \max\left\{\frac 1\ns, \frac{\log \ns}{\ns}\right\},\nonumber\\
& = 2\cdot \frac{\log \ns}{\ns}.
\end{align}

\paragraph{Proof of~\eqref{eq:variance-emp}.}The variance bound of $\frac{\log k}{n}$ is given precisely in~\cite[Lemma 15]{JiaoVHW17}.
To obtain the other half of the bound of, we apply the bounded differences inequality.

\begin{lemma}[BLM-Cor 3.2]
	\label{lem:bdd-diff-var}
	Let $f:\Omega^{\ns}\to\RR$ be a function. Suppose further that 
	\[
	\max_{z_1,\ldots, z_n, z_{i}^{'}} \absv{f(z_1,\ldots,z_n) - f(z_1,\ldots, z_{i-1}, z_i^{'},\ldots,z_n)}\le c_i.
	\]
	Then for independent variables $Z_1,\ldots,Z_{\ns}$, 
	\[
	\Var\Paren{f(Z_1,\ldots,Z_{\ns})} \le \frac14\sum_{i=1}^{\ns} c_i^2.
	\]
\end{lemma}

Therefore, using Lemma~\ref{lem:bdd-diff-var} and Equation~\eqref{eqn:sensitivity-emp}
\[
\variance{\entemp}\le \ns\cdot\Paren{\frac{4\log^2\ns}{\ns^2}} = \frac{4\log^2\ns}{\ns}.
\]

%\begin{theorem}\label{lb:all}
%Any entropy estimator must take 
%\[
%\Omega\Paren{\frac{\ab}{\dist\log\ab}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2}+\frac{\log\ab}{\dist\eps}}
%\]
%samples to estimate $\entp{\p}$ up to $\pm\eps$. Therefore, 
%\[
%\variance{\entemp}\le \ns\cdot\Paren{\frac{4\log^2\ns}{\ns^2}} = \frac{4\log^2\ns}{\ns}.
%\]
%\end{theorem}
%
%As a corollary, note that when $\eps$, and $\dist$ are at most inverse polynomial in $\ab$, then the dependence of the sample complexity is optimal in terms of the privacy parameter. 


==> lb.tex <==
\subsubsection{Lower Bound for Entropy Estimation}

\begin{theorem}\label{lb:all}
\[
C(H, \dist, \eps) =\Omega\Paren{\frac{\ab}{\dist\log\ab}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2}+\frac{\log\ab}{\dist\eps}}.
\]
\end{theorem}
\begin{proof}
The first two terms in the lower bound follows from the entropy estimation lower bounds, even without privacy requirements. For the final term, we will invoke the lower bound arguments from~\cite{AcharyaSZ17}.\todo{Do we need to state the lemma here?} Consider the two distributions below (which are also used in~\cite{WuY16}). The first distribution assigns probability $2/3$ to the first element, and is uniform over the remaining $\ab-1$ elements, and the second distribution assigns probability $(2-\eta)/3$ to the first element, and is uniform over the rest. Then, the entropy of the two distributions differ by $\Theta(\eta\log\ab)$. Therefore, when $\eta = \dist/\log\ab$, the entropy of the two distributions differ by $\Theta(\dist)$. There is a coupling between the two distributions with expected Hamming distance $\expectation{D} = {\eta\ns}/3$. Therefore, 
\[
\eta\ns\ge\frac1\eps \Rightarrow \ns\ge\frac1{\eta\eps}.
\]
Substituting, $\eta = \dist/\log\ab$, gives
\[
\ns\ge \frac{\log\ab}{\dist\eps}.
\]
\end{proof}




==> polynomial.tex <==
\subsubsection{Upper Bound for Entropy Estimation: Best-Polynomial Approximation}
The upper bound should be straightforward from the sensitivity bound in Lemma 2 of~\cite{AcharyaDOS17}.


The optimal sample complexity of estimating $\entp{\p}$ to $\pm \dist$ is~\cite{WuY16}
\[
O\Paren{\frac{\ab}{\dist\log\ab}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2}}.
\]
However, \todo{which two papers?}both these papers propose estimators that can have a high sensitivity.~\cite{AcharyaDOS17} propose technical modifications to these approaches to obtain an estimator that has the following properties. We denote their estimator with $H^\beta$, where $\beta>0$ is a fixed constant (say 0.01 or something).  Then the estimator satisfies the followings:
\begin{itemize}
\item
The sample complexity of the estimator is at most a factor $1/\beta^2$ of the optimal, which is sample order-optimal for any constant $\beta$. 
\item
The sensitivity of $H^{\beta}$ is at most $O(\ns^{\beta}/\ns)$. 
\end{itemize}

This shows the following bound on the sample complexity of estimating $\entp{\p}$ under $\eps$-differential privacy. 
\begin{theorem}
Let $\beta>0$ be a small fixed constant. Then,  
\[
C(H, \dist, \eps) = O\Paren{\frac{\ab}{\beta^2\dist\log\ab}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2} + \Paren{\frac1{\dist\eps}}^{1+\beta}}.
\]
which can estimate $\entp{\p}$ up to $\pm \dist$ with success probability of 2/3.
\end{theorem}




